Background estimation in the search for single production of vector-like quarks decaying into $Wb$ in $pp$ collisions using a data-driven method at $\sqrt{s} = 13$ TeV with the ATLAS detector

A search for singly produced vector-like $T/Y$ quark is performed in proton-proton collision data at a centre-of-mass energy of $13$ TeV corresponding to an integrated luminosity of $139.1 fb^{-1}$, recorded with the ATLAS detector at the LHC from 2015-18. The analysis focused on the hadronic channel of $T/Y \rightarrow Wb$ decay mode. The hadronic channel is not a clean channel, unlike the leptonic channel, because of the contribution coming from the QCD processes, which accounts for a significant background. The modelling of QCD processes is challenging due to their theoretical prediction and experimental challenges. Due to this, it is observed that the Monte Carlo simulation of the QCD multijet is mismodelled in this analysis. In this thesis, a data-driven method called the ABCD method is presented to estimate the QCD multijet background. The method uses the background events from all the control regions to estimate the multijets in the signal region. However, a correlation among different control regions is observed, which is further accounted by introducing a correlation factor. The correlation factor is calculated by performing likelihood fit to the MC simulated backgrounds. Some additional studies, including uncertainty estimation on the method and the performance of the method with different jet collections and taggers, are also performed.

==> Makefile <==
# Makefile to run latex, dvips, and pdflatex on a thesis
# Can also run feynmf/feynmp/tikz on files in a directory

THESIS = mythesis
# EXTRACMD = --shell-escape
FEYNDIR = feynmf
FEYNFILES = $(wildcard $(FEYNDIR)/*.tex)
TIKZDIR = tikz
TIKZFILES = $(wildcard $(TIKZDIR)/*.tex)
PYFEYNDIR = pyfeyn
PYFEYNFILES = $(wildcard $(PYFEYNDIR)/*.py)
ifdef file
FEYNFILES = $(FEYNDIR)/$(file).tex
TIKZFILES = $(TIKZDIR)/$(file).tex
PYFEYNFILES = $(PYFEYNDIR)/$(file).py
endif
BIBTEX = biber
AWKDIR=..

.PHONY: cover \
	feynmf feynmp tikz pyfeyn \
	cleanthesis cleancover \
	cleanfeynmf cleanfeynmp cleantikz cleanpyfeyn cleanpictpdf \
	cleanblx cleanbbl \
	cleanglo cleanlatexmk\
	help test

thesis: run_latexmk

# Use latexmk to compile thesis
run_latexmk:  $(THESIS).tex *.tex bib/*.bib
	latexmk -pdf $(THESIS)
	# LATEXMK = latexmk -e '$$pdflatex=q/pdflatex %O -shell-escape %S/' -pdf $(THESIS)

# - in front of bibtex means compilation continues even if there is an error
thesis09: $(THESIS).tex *.tex bib/*.bib
	pdflatex   $(EXTRACMD) $(THESIS)
	-bibtex $(THESIS)
	# makeglossaries $(THESIS)
	pdflatex   $(EXTRACMD) $(THESIS)
	pdflatex   $(EXTRACMD) $(THESIS)

thesis11: $(THESIS).tex *.tex bib/*.bib
	pdflatex   $(EXTRACMD) $(THESIS)
	$(BIBTEX)  $(THESIS)
	# makeglossaries $(THESIS)
	pdflatex   $(EXTRACMD) $(THESIS)
	pdflatex   $(EXTRACMD) $(THESIS)

cover:
	pdflatex   $(EXTRACMD) cover_only
	pdflatex   $(EXTRACMD) cover_only

feynmf:
	make -f ../Makefile FEYNDIR=$(FEYNDIR) FEYNFILES="$(FEYNFILES)" \
	 AWKDIR=$(AWKDIR) feynmf

feynmp:
	make -f ../Makefile FEYNDIR=$(FEYNDIR) FEYNFILES="$(FEYNFILES)" \
	 AWKDIR=$(AWKDIR) feynmp

tikz:
	make -f ../Makefile TIKZDIR=$(TIKZDIR) TIKZFILES="$(TIKZFILES)" tikz

pyfeyn:
	make -f ../Makefile PYFEYNDIR=$(PYFEYNDIR) PYFEYNFILES="$(PYFEYNFILES)" pyfeyn

thesis_feynmf:
	feynmf $(THESIS)

cleanall: clean cleanbbl cleanpictpdf

clean: cleanthesis cleancover \
	cleanfeynmf cleanfeynmp cleantikz \
	cleanblx cleanglo cleanlatexmk

cleanthesis:
	-rm $(THESIS).log $(THESIS).aux $(THESIS).toc
	-rm $(THESIS).lof $(THESIS).lot $(THESIS).out
	-rm $(THESIS).blg $(THESIS).bbl $(THESIS).pdf
	-rm $(THESIS).fdb_latexmk .$(THESIS).lb $(THESIS).synctex.gz
	-rm *.aux

cleancover:
	-rm cover_only.log cover_only.aux cover_only.out
	-rm cover_only.pdf

cleanfeynmf:
	-rm *.mf *.tfm *.t1 *.600gf *.600pk *.log
	-rm feynmf_all.* feynmf_files.inp

cleanfeynmp:
	-rm *.1 *.log *.mp *.t1
	-rm feynmf_all.* feynmf_files.inp

cleantikz:
	-rm $(TIKZDIR)/*.log $(TIKZDIR)/*.aux

cleanpyfeyn:
	-rm $(PYFEYNDIR)/*.pdf

cleanpictpdf:
	-rm $(FEYNDIR)/*.pdf
	-rm $(TIKZDIR)/*.pdf
	-rm $(PYFEYNFDIR)/*.pdf

cleanblx:
	-rm *-blx.bib
	-rm *.bcf
	-rm *.run.xml

cleanbbl:
	-rm *.bbl

cleanglo:
	-rm *.acn *.acr *.alg
	-rm *.glg *.glo *.gls
	-rm *.ist

cleanlatexmk:
	-rm *.fdb_latexmk *.fls

help:
	@echo "Possible commands:"
	@echo "new [THESIS=dirname]: Set up a new thesis"
	@echo "thesis: Compile complete thesis (latexmk)"
	@echo "run_latexmk: Compile complete thesis using latexmk"
	@echo "thesis11: Compile complete thesis - texlive >=2011 + biber"
	@echo "thesis09: Compile complete thesis - texlive 2009 + bibtex"
	@echo "feynmf: Run feynmf for all .tex files in $(FEYNDIR)"
	@echo "feynmp: Run feynmp for all .tex files in $(FEYNDIR)"
	@echo "tikz:   Run tikz for all .tex files in $(TIKZDIR)"
	@echo "clean:         Clean up most auxiliary files (leaves bbl and picture PDF files)"
	@echo "cleanall:      Clean up all auxiliary files"
	@echo "cleanthesis:   Clean up thesis LaTeX output files"
	@echo "cleanbbl:      Clean up thesis bbl files"
	@echo "cleanblx:      Clean up thesis biber files"
	@echo "cleanfeynmf:   Clean up feynmf output files"
	@echo "cleantikz:     Clean up tikz temparary files"
	@echo "cleanpyfeyn:   Clean up pyfeyn PDF files"
	@echo "cleanpictpdf:  Clean up picture output in $(FEYNDIR), $(TIKZDIR) and $(PYFEYNDIR)"
	@echo "cleanglo:      Clean up glossary output files"
	@echo "cleanlatexmk:  Clean up latexmk files"

test:
	@echo "Thesis $(THESIS)"
	@echo "Feynmf Feynman graphs dir: $(FEYNDIRNAME)"
	@echo "Feynmf Feynman graphs files: $(FEYNFILES)"
	@echo "TikZ   Feynman graphs dir: $(TIKZDIRNAME)"
	@echo "TikZ   Feynman graphs files: $(TIKZFILES)"
	@echo "PyFeyn Feynman graphs dir: $(PYFEYNDIRNAME)"
	@echo "PyFeyn Feynman graphs files: $(PYFEYNFILES)"


==> README <==
Version 6.0 08/12/2018

The idea with this package is that you also look at the LaTeX that
is used to create it, in order to find out how things are done.

The files that make up this package are available in a git
repository and as a tar file. To get the latest subversion
entries given the command:

git clone https://git.physik.uni-bonn.de/cgit/projects/ubonn-thesis.git

If you want a particular release use the command:

git clone --branch v6.0 https://git.physik.uni-bonn.de/cgit/projects/ubonn-thesis.git

The tar file also includes the guide as a PDF file: guide/thesis_guide.pdf.
It can be obtained from:

https://www.pi.uni-bonn.de/lehre/uni-bonn-thesis

You can give the command:

make new [THESIS=dirname] [TEXLIVE=YYYY]

to create a new directory with a few files to help you get
started. By default the directory name will be mythesis.
To compile your thesis try:

cd mythesis [or dirname]
make thesis

All packages that are needed should be part of your TeX
installation. If not you may have to install them or ask your system
administrator to do so.

My original idea was that the style file should work for all recent
TeX installations.  However, some of the packages I recommend have
been changing quite a lot over the past few years, particularly
biblatex and siunitx.  It may therefore be necessary to make a few
changes in order to get the thesis to compile on your machine. The
default version assumes that you have TeX Live 2013 or later.  If you
have an older version pass the option 'texlive=YYYY' to the document class
or ubonn-thesis package in mythesis.tex.
If you make a new document, you can do this by passing the argument 
`TEXLIVE=YYYY' when giving the command `make new'.

If your version of TeX Live is earlier than 2011, which implies that you have
siunitx version 1 and that you use bibtex8 with biblatex,
you should use the command `make thesis09' instead of `make thesis' in order to compile.
You can use the command 'make new09' to make a thesis skeleton suitable for use with
TeX Live 2009. This version also uses traditional BibTeX by default.

If you just want to make the cover pages, use the file cover_only.tex.
Be sure to adapt the font selected in ubonn-thesis.sty to the font
you actually used in your thesis. Be aware that not all font sizes are
available in all font collections. If you used the default LaTeX font
in your thesis, then choose lmodern in the style file.

The main file for this guide is guide/thesis_guide.tex and it
includes the LaTeX files in the directory ./guide and the
Feynman graphs in the directories ./feynmf and ./tikz.

You can create your own copy of the guide using the commands:

cd guide
make guide

If you have a version of TeX Live older than 2013, you should set 
\texlive appropriately thesis_guide.tex and
should not pass the newtx option to ubonn-thesis.
If your version of TeX Live is older than 2011, you need to compile the 
guide with the commands `make feynmf; make guide09' instead of `make guide'.

The guide also includes a description of how to use the package under
Windows.


==> awk_feynmp <==
/begin.*fmfgraph/ {gsub(/[\{\}(),]/," "); print $3; print $4}


==> cover/Bachelor_Title.tex <==
%
% Title page layout for submitted version
%
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\LARGE
  \begin{otherlanguage}{ngerman}
    Bachelorarbeit in Physik\\
    angefertigt \inInstitute\\[3ex]
    vorgelegt der\\
    Mathematisch-Naturwissenschaftlichen Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität\\
    Bonn\\[3ex]
    \thesismonth{} \thesisyear
  \end{otherlanguage}
  \vspace*{\fill}
}
\lowertitleback{%
  \begin{otherlanguage}{ngerman}
    Ich versichere, dass ich diese Arbeit selbstständig
    verfasst und keine anderen als die angegebenen Quellen und
    Hilfsmittel benutzt sowie die Zitate kenntlich gemacht habe.

    \vspace*{4ex minus 0.5ex}

    \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
      Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
      & Datum & Unterschrift
    \end{tabular}
  \end{otherlanguage}

  % \begin{otherlanguage}{UKenglish}
  %   I hereby declare that this thesis was formulated by
  %   myself and that no sources or tools other than those cited were used.

  %   \vspace*{4ex minus 0.5ex}

  %   \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
  %     Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
  %     & Date & Signature
  %   \end{tabular}
  % \end{otherlanguage}

  \vspace*{10ex minus 4ex}

  \noindent
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{@{}ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> cover/Diplom_Cover.tex <==
%
% Cover page layout for the department library version
%
% Make the top margin on the title page larger and also increase the
% size of the left margin to allow for binding. These parameters may
% have to be adjusted if you change the fraction of the page area that
% is used for the text.
% Changing margins works well. Changing the text height has a bad
% effect on the table of contents.
%
{\thispagestyle{empty}
  \addtolength{\oddsidemargin}{1.0cm}\addtolength{\topmargin}{1.0cm}
  \rmfamily\setlength{\parindent}{0pt}
  \begin{center}
    {\fontsize{44}{50}\selectfont
      Universität Bonn}

    \vspace*{20pt}

    \begin{singlespace}
      \fontsize{30}{40}\selectfont
      \InstituteName
    \end{singlespace}

    \vspace*{40pt}

    \begin{onehalfspace}
      \bfseries\huge
      \thesistitle
    \end{onehalfspace}

    \vspace*{20pt}

    {\huge
      \thesisauthor
    }
  \end{center}

  \vspace*{\fill}

  \thesisabstract

  \vspace*{\fill}

  {\normalfont\normalsize
    \parbox{0.3\textwidth}{\InstituteAddress}
    \parbox{0.4\textwidth}{%
      \centering
      \includegraphics[width=5cm]{instituts_siegel}
    }
    \parbox{0.3\textwidth}{%
      \thesisnumber\\
      \thesismonth{} \thesisyear
    }
  }
}


==> cover/Diplom_Final_Title.tex <==
%
% Title page layout for printed version
%
\titlehead{%
  \centering
  {\fontsize{44}{50}\selectfont
    Universität Bonn}

  \vspace*{20pt}

  \begin{singlespace}
    \fontsize{30}{40}\selectfont
    \InstituteName
  \end{singlespace}
}
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\vspace*{\fill}
  \raggedright
  {\normalsize
    \begin{otherlanguage}{ngerman}
      Dieser Forschungsbericht wurde als Diplomarbeit von der
      Mathematisch-Naturwissenschaftlichen Fakultät der Universität Bonn
      angenommen.
    \end{otherlanguage}

    \vspace*{10ex minus 4ex}

    \noindent
    \begin{tabular}{@{}ll}
      Angenommen am:         & \thesissubmit\\
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  }
}

\maketitle


==> cover/Diplom_Submit_Title.tex <==
%
% Title page layout for submitted version
%
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\LARGE
  \begin{otherlanguage}{ngerman}
    Diplomarbeit in Physik\\
    angefertigt \inInstitute\\[3ex]
    vorgelegt der\\
    Mathematisch-Naturwissenschaftlichen Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität\\
    Bonn\\[3ex]
    \thesismonth{} \thesisyear
  \end{otherlanguage}
  \vspace*{\fill}
}
\lowertitleback{%
  \begin{otherlanguage}{ngerman}
    Ich versichere, dass ich diese Arbeit selbstständig
    verfasst und keine anderen als die angegebenen Quellen und
    Hilfsmittel benutzt sowie die Zitate kenntlich gemacht habe.

    \vspace*{4ex minus 0.5ex}

    \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
      Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
      & Datum & Unterschrift
    \end{tabular}
  \end{otherlanguage}

  % \begin{otherlanguage}{UKenglish}
  %   I hereby declare that this thesis was formulated by
  %   myself and that no sources or tools other than those cited were used.

  %   \vspace*{4ex minus 0.5ex}

  %   \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
  %     Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
  %     & Date & Signature
  %   \end{tabular}
  % \end{otherlanguage}

  \vspace*{10ex minus 4ex}

  \noindent
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{@{}ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> cover/Guide_Submit_Title.tex <==
% chktex-file 21

% Title page layout for submitted version.
\title{\thesistitle}
\subtitle{\vspace*{4ex}
  \begin{otherlanguage}{ngerman}
    Hinweise und Tipps\\
    zur\\
    Produktion einer Bachelor/Master/Diplom/Doktorarbeit\\
    in der\\
    Mathematisch-Naturwissenschaftlichen-Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität Bonn
  \end{otherlanguage}
}
\author{%
  vorgelegt von\\
  \thesisauthor\\
  aus\\
  \thesistown%
}
\date{Version \guideversion\\
  \today}
\publishers{%
  Bonn \thesisyear%
}
\lowertitleback{%
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo\\[2ex]
      Tag der Promotion: & \\
      Erscheinungsjahr: & 
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> cover/Master_Cover.tex <==
%
% Cover page layout for the department library version
%
% Make the top margin on the title page larger and also increase the
% size of the left margin to allow for binding. These parameters may
% have to be adjusted if you change the fraction of the page area that
% is used for the text.
% Changing margins works well. Changing the text height has a bad
% effect on the table of contents.
%
{\thispagestyle{empty}
  \addtolength{\oddsidemargin}{1.0cm}\addtolength{\topmargin}{1.0cm}
  \rmfamily\setlength{\parindent}{0pt}
  \begin{center}
    {\fontsize{44}{50}\selectfont
      Universität Bonn}

    \vspace*{20pt}

    \begin{singlespace}
      \fontsize{30}{40}\selectfont
      \InstituteName
    \end{singlespace}

    \vspace*{40pt}

    \begin{onehalfspace}
      \bfseries\huge
      \thesistitle
    \end{onehalfspace}

    \vspace*{20pt}

    {\huge
      \thesisauthor
    }
  \end{center}

  \vspace*{\fill}

  \thesisabstract

  \vspace*{\fill}

  {\normalfont\normalsize
    \parbox{0.3\textwidth}{\InstituteAddress}
    \parbox{0.4\textwidth}{%
      \centering
      \includegraphics[width=5cm]{instituts_siegel}
    }
    \parbox{0.3\textwidth}{%
      \thesisnumber\\
      \thesismonth{} \thesisyear
    }
  }
}


==> cover/Master_Final_Title.tex <==
%
% Title page layout for printed version
%
\titlehead{%
  \centering
  {\fontsize{44}{50}\selectfont
    Universität Bonn}

  \vspace*{20pt}

  \begin{singlespace}
    \fontsize{30}{40}\selectfont
    \InstituteName
  \end{singlespace}
}
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\vspace*{\fill}
  \raggedright
  {\normalsize
    \begin{otherlanguage}{ngerman}
      Dieser Forschungsbericht wurde als Masterarbeit von der
      Mathematisch-Naturwissenschaftlichen Fakultät der Universität Bonn
      angenommen.
    \end{otherlanguage}

    \vspace*{10ex minus 4ex}

    \noindent
    \begin{tabular}{@{}ll}
      Angenommen am:         & \thesissubmit\\
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  }
}

\maketitle


==> cover/Master_Submit_Title.tex <==
%
% Title page layout for submitted version
%
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\LARGE
  \begin{otherlanguage}{ngerman}
    Masterarbeit in Physik\\
    angefertigt \inInstitute\\[3ex]
    vorgelegt der\\
    Mathematisch-Naturwissenschaftlichen Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität\\
    Bonn\\[3ex]
    \thesismonth{} \thesisyear
  \end{otherlanguage}
  \vspace*{\fill}
}
\lowertitleback{%
  % \begin{otherlanguage}{ngerman}
  %   Ich versichere, dass ich diese Arbeit selbstständig
  %   verfasst und keine anderen als die angegebenen Quellen und
  %   Hilfsmittel benutzt sowie die Zitate kenntlich gemacht habe.

  %   \vspace*{4ex minus 0.5ex}

  %   \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
  %     Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
  %     & Datum & Unterschrift
  %   \end{tabular}
  % \end{otherlanguage}

  \begin{otherlanguage}{UKenglish}
    I hereby declare that this thesis was formulated by
    myself and that no sources or tools other than those cited were used.

    \vspace*{4ex minus 0.5ex}

    \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
      Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
      & Date & Signature
    \end{tabular}
  \end{otherlanguage}

  \vspace*{10ex minus 4ex}

  \noindent
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{@{}ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> cover/PhD_Cover.tex <==
%
% Cover page layout for the department library version
%
% Make the top margin on the cover page larger and also increase the
% size of the left margin to allow for binding. These parameters may
% have to be adjusted if you change the fraction of the page area that
% is used for the text.
% Changing margins works well. Changing the text height has a bad
% effect on the table of contents.
%
{\thispagestyle{empty}
  \addtolength{\oddsidemargin}{1.0cm}\addtolength{\topmargin}{1.0cm}
  \rmfamily\setlength{\parindent}{0pt}
  \begin{center}
    {\fontsize{44}{50}\selectfont
      Universität Bonn}

    \vspace*{20pt}

    \begin{singlespace}
      \fontsize{30}{40}\selectfont
      \InstituteName
    \end{singlespace}

    \vspace*{40pt}

    \begin{onehalfspace}
      \bfseries\huge
      \thesistitle
    \end{onehalfspace}

    \vspace*{20pt}

    {\LARGE
      \thesisauthor
    }
  \end{center}

  \vspace*{\fill}

  \thesisabstract

  \vspace*{\fill}

  {\normalfont\normalsize
    \parbox{0.3\textwidth}{\InstituteAddress}
    \parbox{0.4\textwidth}{%
      \centering
      \includegraphics[width=5cm]{instituts_siegel}
    }
    \parbox{0.3\textwidth}{%
      \thesisnumber\\
      \thesismonth{} \thesisyear\\
      ISSN-0172-8741
    }
  }
}


==> cover/PhD_Final_Title.tex <==
%
% Title page layout for published version
%
% \titlehead{%
%   \centering
%   {\fontsize{44}{50}\selectfont
%     Universität Bonn}

%   \vspace*{20pt}

%   \begin{singlespace}
%     \fontsize{30}{40}\selectfont
%     \InstituteName
%   \end{singlespace}
% }
\title{\thesistitle}
\subtitle{\vspace*{4ex}
  \begin{otherlanguage}{ngerman}
    Dissertation\\
    zur\\
    Erlangung des Doktorgrades (Dr.\ rer.\ nat.)\\
    der\\
    Mathematisch-Naturwissenschaftlichen Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität Bonn
  \end{otherlanguage}
}
\author{%
  von\\
  \LARGE \thesisauthor\\
  aus\\
  \thesistown
}
\date{}
\publishers{%
  Bonn, \thesissubmit
}
\lowertitleback{\normalsize
  \raggedright
  \begin{otherlanguage}{ngerman}
    Dieser Forschungsbericht wurde als Dissertation von der
    Mathematisch-Naturwissenschaftlichen Fakultät der Universität
    Bonn angenommen und ist auf dem
    Hochschulschriftenserver der ULB Bonn
    \url{http://hss.ulb.uni-bonn.de/diss_online} elektronisch
    publiziert.
  \end{otherlanguage}

  \vspace*{10ex minus 4ex}

  \noindent
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo\\[2ex]
      Tag der Promotion: & \thesispromotion\\
      Erscheinungsjahr: & \thesisyear
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> cover/PhD_Submit_Title.tex <==
%
% Title page layout for submitted version.
%
\title{\thesistitle}
\subtitle{\vspace*{4ex}
  \begin{otherlanguage}{ngerman}
    Dissertation\\
    zur\\
    Erlangung des Doktorgrades (Dr.\ rer.\ nat.)\\
    der\\
    Mathematisch-Naturwissenschaftlichen Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität Bonn
  \end{otherlanguage}
}
\author{%
  vorgelegt von\\
  \thesisauthor\\
  aus\\
  \thesistown
}
\date{}
\publishers{%
  Bonn \thesisyear
}
\lowertitleback{\normalsize
  \begin{otherlanguage}{ngerman}
    Angefertigt mit Genehmigung der 
    Mathematisch-Naturwissenschaftlichen Fakultät der
    Rheinischen Friedrich-Wilhelms-Universität Bonn
  \end{otherlanguage}
  
  \vspace*{10ex minus 4ex}
  
  \noindent
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{@{}ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo\\[2ex]
      Tag der Promotion:      & \\
      Erscheinungsjahr:       & 
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> cover_test/Makefile <==
#
# Makefile to run pdflatex on different covers
#
# EXTRACMD = --shell-escape

.PHONY: cover_test
	cleancover \
	help test

cover_test:
	pdflatex  $(EXTRACMD) cover_test
	biber cover_test
	pdflatex  $(EXTRACMD) cover_test

cleanall: clean

clean: cleancover

cleancover:
	-rm cover_test.log cover_test.aux cover_test.toc cover_test.out
	-rm cover_test.bcf cover_test.run.xml
	-rm cover_test.blg cover_test.bbl cover_test.pdf

help:
	@echo "Possible commands:"
	@echo "cover_test: Test covers"
	@echo "cleancover: Clean up cover test files"

test:
	@echo "Nothing to test!"


==> run_mf <==
#! /bin/sh
#
# Script to run mf locally in directory given in filename
#
if [ $# -le 0 ]; then
   echo "Must give filename"
   exit 1
fi
#
# if [ ! -f $1 ]; then
#    echo "File $1 does not exist"
#    exit 1
# fi
#
dir=`dirname $1`
file=`basename $1 .tex`
#
# Do not process files that start with feynmf_
#
# echo $file | grep "^feynmf_" && exit
#
echo "Directory: <$dir>"
echo "File: <$file>"
# cd $dir
mf "\mode=localfont; input $file"


==> thesis_acknowledge.tex <==
%------------------------------------------------------------------------------
\chapter{Acknowledgements}
\label{sec:acknowledgements}
%------------------------------------------------------------------------------
In 2017, I had the fortune to come to Germany and study physics. This would not have been possible without Bonn-Cologne Graduate School, so I would like to thank the admission committee for giving me an opportunity to pursue my master degree in physics.

I would like to thank Prof.\ Dr.\ Ian C.\ Brock for giving me an opportunity to write my thesis in his group. There is no doubt that without his guidance, wisdom and direction over the course of my degree, this thesis would not have been possible. I would also like to thank Prof.\ Dr.\ Florian Bernlochner, who agreed to be my second referee for this thesis.

Furthermore, I would like to thank Prof.\ Dr.\ Heiko Lacker, Dr.\ Janet Dietrich and Ferdinand Schenck from the Berlin VLQ group for helping me to understand the analysis better and also for their fruitful discussions on my results.

A big thanks to Anjishnu Bandyopadhyay for his support right from the beginning, when he introduced me VLQs till the last day of my submission. I truly appreciate all of his efforts for helping me with all my queries irrespective of the time on the clock as well as the priceless discussions on physics-related topics during DPG and at CERN. It has been a pleasure working with him. I would also like to thank Dr.\ Regina Moles Valls and Dr.\ Rui Zhang for their guidance and motivation when I initially joined this group as an intern. I would like to thank Dr.\ Oleh Kivernyk for his valuable suggestions on my results on the ABCD method.

Next, I would like to thank Federico G.\ D.\ Capriles for proofreading my first draft of this thesis and giving me some good memories of card game evenings. I would also like to thank Tanja Holm for the priceless discussions on jets and Christian Kirfel for the general discussions on machine learning related topics as well as teaching me some basic German culture. I would also like to thank Chris Boever for always motivating me and constantly reminding me that I am the next one after him. I am also grateful to him for proofreading some parts of my first draft of this thesis. I would like to thank Hanna We for all the interesting discussions we had on Indian and Korean cultures while sharing the same office. A special thanks to all the other members of the Brock group who were in the group during my days there, including but not limited to Nilima, Nicolas, Piet, Ellinor, Richard.

I would also like to thank everyone in the Desch group for the discussions during the Jamborees. A special thanks to all my friends and colleagues without them, my experience during my degree would not be as enjoyable.

Finally, I would like to thank my parents and family who are \SI{6000}{\kilo\meter} away from me but still their unconditional love and unlimited support encouraged me to start my venture; without them, it would not have been possible for me to manage and finish my studies.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../mythesis"
%%% End: 


==> thesis_cv.tex <==
\definecolor{lightgray}{gray}{0.8}
\newcolumntype{L}{>{\raggedleft}p{0.15\textwidth}}
\newcolumntype{R}{p{0.8\textwidth}}
\newcommand\VRule{\color{lightgray}\vrule width 0.5pt}

\thispagestyle{empty}
\section*{Curriculum Vitae}

\subsection*{Personal Details}

\begin{tabular}{L!{\VRule}R}
Name & Johann Schmidt \\
Date of Birth &  \\
Email & abc@physik.uni-def.de \\
Family status & Single
\end{tabular}

\subsection*{Education}

\begin{tabular}{L!{\VRule}R}
1997--2003 & Abitur, ABC Secondary School, Hamburg, Germany\\
2004--2007 & BSc in Physics, Rheinische Friedrich-Wilhelms-Universität, Bonn, Germany.\\
2006 & CERN Summer Student, Geneva, Switzerland. \\
2007--2009 &  MSc in Physics Rheinische Friedrich-Wilhelms-Universität, Bonn, Germany. \\
2009--2012 &  PhD in Physics, Rheinische Friedrich-Wilhelms-Universität, Bonn, Germany. \\
2012 & Advanced Data Analysis School, Frankfurt, Germany.
\end{tabular}

\subsection*{Professional Experience}

\begin{tabular}{L!{\VRule}R}
2004 & Summer Student at CERN, Geneva, Switzerland. \\
2007--2012 & Doctoral work at the University of Bonn, Germany. \\
2008--2009 & Fieldwork at CERN, Geneva, Switzerland.\\
2011 & Talk at the Advanced Physics Conference, Timbucto
\end{tabular}

\subsection*{Languages}
\begin{tabular}{L!{\VRule}R}
German & Mother tongue \\
English & Fluent \\
Russian & Basic
\end{tabular}

